Re-evaluation of the LHC potential for the measurement of Mw

We present a study of the LHC sensitivity to the W boson mass based on simulation studies. We find that both experimental and phenomenological sources of systematic uncertainties can be strongly constrained with Z measurements: the lineshape is robustly predicted, and its analysis provides an accurate measurement of the detector resolution and absolute scale, while the differential cross-section analysis absorbs most of the strong interaction uncertainties. A sensitivity $\delta Mw \sim 7 \MeV$ for each decay channel (W --> e nu, W --> mu nu), and for an integrated luminosity of 10 fb-1, appears as a reasonable goal.

==> definitions.tex <==
\newcommand{\W}{\ensuremath{W}\xspace}
\newcommand{\Wpm}{\ensuremath{W^{\pm}}\xspace}
\newcommand{\Z}{\ensuremath{Z}\xspace}
\newcommand{\Zzero}{\ensuremath{Z^0}\xspace}       % I don't use this one
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}

\newcommand{\pt}{\ensuremath{p_t}\xspace}
\newcommand{\ptl}{\ensuremath{p_t^l}\xspace}
\newcommand{\pte}{\ensuremath{p_t^e}\xspace}
\newcommand{\ptlp}{\ensuremath{p_t(l)}\xspace}
\newcommand{\ptn}{\ensuremath{p_t^\nu}\xspace}
\newcommand{\ptw}{\ensuremath{p_t^W}\xspace}
\newcommand{\mw}{\ensuremath{m_W}\xspace}
\newcommand{\mtw}{\ensuremath{m_t^W}\xspace}
\newcommand{\dmw}{\ensuremath{\delta m_W}\xspace}
\newcommand{\mtwp}{\ensuremath{m_t(W)}\xspace}

\newcommand{\yw}{\ensuremath{y_W}\xspace}
\newcommand{\yz}{\ensuremath{y_Z}\xspace}

\newcommand{\met}{\ensuremath{E_t \hspace*{-3.0ex} \not~~}\xspace}
\newcommand{\etmiss}{\ensuremath{E_t \hspace*{-3.0ex}  \not~~}\xspace}
 
\newcommand{\ptvl}{\ensuremath{\vec{p}_t^l}\xspace}
\newcommand{\etl}{\ensuremath{E_t^l}\xspace}
\newcommand{\ptvn}{\ensuremath{\vec{p}_t^\nu}\xspace}
\newcommand{\etn}{\ensuremath{E_t^\nu}\xspace}

\newcommand{\pb}{\ensuremath{\mbox{\,pb}}\xspace}
\newcommand{\invpb}{\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\newcommand{\fb}{\ensuremath{\mbox{\,fb}}\xspace}
\newcommand{\invfb}{\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\newcommand{\lumi}{\ensuremath{\cal L}\xspace}
 


==> ratiomethod.tex <==

%% A popular measurement method, previously employed at the
%% Tevatron~\cite{} and envisaged by the CMS collaboration~\cite{},
%% consists of directly deducing W observables from Z ones, after a
%% simple phase space rescaling: 
%% 
%% \begin{equation}
%% \frac{d\sigma_W}{dO_W}\left(O_W\right) \equiv \frac{M_Z}{M_W} R\left(\frac{O_W}{M_W}\right) 
%% %%       \frac{d\sigma_Z}{dO_Z}\left(O_Z = \frac{M_Z}{M_W} O_W\right),
%% \label{eq:ratio}
%% \end{equation}
%% 
%% \noindent where $O$ is an observable measured in W and Z events (e.g,
%% \ptl), the $Z$ differential cross-section is to be measured in the
%% data, and the $W$ differential cross-section is deduced as a result of
%% the above formula.
%% 
%% We insist that this formalism can not be employed as such at the
%% LHC. Indeed, a built-in assumption is that the $W$ phase space can be
%% deduced from the $Z$ one by a simple rescaling factor ($M_W /
%% M_Z$). This however poses problems, because the $W$ width needs to be
%% measured $per$~$se$, and in any case is not equal to the scaled $Z$ width: 
%% 
%% \begin{eqnarray}
%% \Gamma_W \ne \frac{M_W}{M_Z} \,\, \Gamma_Z.
%% \label{eq:scaledwidth}
%% \end{eqnarray}

%% Hence, a measurement based on Eq.~\ref{eq:ratio} will carry
%% an intrinsic bias, coming from the approximate mapping of the $Z$
%% phase space into the $W$ one. Given the expected statistics, this
%% bias should be prohibitive.

As illustrated by this paper, the measurement of \MW\ at the LHC
relies on auxiliary measurement to constrain almost all relevant
uncertainties, both experimental and phenomenological.

The auxiliary measurements are in general performed using process that
have different centre-of-mass energy ($\hat{s}$) distributions than the
target process, i.e. W production. This is certainly the case of the
neutral current processes, Z production and off-peak Drell-Yan events,
used throughout this study.

Where applicable, the $\hat{s}$ dependence of the systematics sources
need to be appropriately folded into the $W$ sample. This would
mean, for an observable $O$:

\begin{itemize}
\item measure the distribution of $O$ as a function of
$\hat{s}$, given by the dilepton invariant mass, in neutral current
events. The invariant mass range needs to comfortably include the W
resonance, to be hypothesized below;
\item for a given hypothesis on the $W$ resonance parameters ($M_W$,
$\Gamma_W$), produce the expected $W$ lineshape, using a full event
generator, as the proton parton density effects need to be properly
accounted for;
\item deduce the distribution of $O$ for $W$ events as
an integral over the $W$ resonance, of $O(\hat{s})$ as measured in
neutral current events. 
\end{itemize}

\noindent This would give:
\begin{equation}
\frac{d\sigma_W}{dO}(O; M_W, \Gamma_W) \equiv R_{th}
\int_{\Delta\hat{s}} d\hat{s} \,\,
      f(\hat{s}; M_W, \Gamma_W) \,\, \frac{d\sigma_{NC}}{dO}(O; \hat{s}),
\end{equation}
\noindent where $R_{th}$ accounts for residual effects, computed
theoretically; $f(\hat{s}; M_W, \Gamma_W)$ represents the $W$
lineshape, for a given mass and width hypothesis, and $\Delta\hat{s}$
is the region over which $f$ is non-zero. 


As we saw in Section~\ref{subsec:systqcd}, this procedure seems
mandatory when accounting for the effects related to $p_T(W)$, for
example. 


